A Transient Queueing Analysis under Time-varying Arrival and Service Rates for Enabling Low-Latency Services

Understanding the detailed queueing behavior of a networking session is critical in enabling low-latency services over the Internet. Especially when the packet arrival and service rates at the queue of a link vary over time and moreover when the session is short-lived, analyzing the corresponding queue behavior as a function of time, which involves a transient analysis, becomes extremely challenging. In this paper, we propose and develop a new analytical framework that anatomizes the transient queue behavior under time-varying arrival and service rates even under unstable conditions. Our framework is capable of answering key questions in designing low-latency services such as the time-dependent probability distribution of the queue length; the instantaneous or time-averaged violation probability that the queue length exceeds a certain threshold; and the fraction of time during an interval $[0, t]$ at which the queue length exceeds a certain threshold. We validate our framework by comparing its prediction results over time with the statistical simulation results and confirm that our analysis is accurate enough. Our extensive demonstrations on the efficacy of the analytical framework in designing low-latency services reveal that its prediction ability for the transient queue behavior in diverse time-varying packet arrival and service patterns can be of a high practical value.

==> system.tex <==
\pdfoutput=1
\section{System}
\label{sec:system}

In this section, we describe the settings of the queueing system that we analyze throughout this paper. %and clarify the problem we focus on solving. 
Then, we interpret the system %as well as its settings
in the perspective of low-latency Internet applications. 

\subsection{System Model}
We target to analyze a generalized single server FIFO queueing system in which its packet arrival and departure conform to Poisson processes and its average arrival rate changes at every rate switching interval whose durations are of constants. For simplicity, we assume that the average departure rate of the system remains the same over time. This system model is depicted in Fig.\ref{fig:system}, where the average arrival rate $\lambda$ switches to a different value at every switching interval $T_i$, while the average departure rate $\mu$ is constant. 

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.95\columnwidth]{figs/system.pdf}
    \caption{The average arrival and departure rate behaviors of a generalize single server queueing system of our interest. The arrival rate changes at every switching interval.}	
    \label{fig:system}
\end{figure}

We clarify here that we aim at developing an analysis framework that can even deal with the queue bubbling case: $\lambda_k > \mu$ where $\lambda_k$ denotes the $\lambda$ during the interval $T_k$, which is known intractable by any steady-state analysis.

%\subsection{Problem Statement}

\subsection{Applications}
Our analysis framework can be useful in many areas, but in this work we give our special attention to low-latency Internet applications, where the question, \textit{can the queueing latency be bounded or not?}, is most critical. In order to emulate general traffic generation behaviors of low-latency applications, we propose two simplified $\lambda_k$ evolution models and perform in-depth studies for such models. Those two models are as follows. 

\noindent{\bf{On and Off Traffic Generation Model:}}
With this model, we emulate the case where a low-latency service user gives timely control toward a remote machine such as a Drone or a self-driving vehicle. Because the control packets are generated intermittently and there exist alternating periods of no control, the packet arrival toward the queueing system from the controlling user resembles alternating on and off periods as shown in Fig.~\ref{fig:caseonoff}. We here note that even when there is no other competing flows in the queueing system, this intermittent packet burst itself builds up the queue and makes a portion of succeeding packets to violate the latency requirement. This is so called, \textit{self-induced queueing}, which is well analyzed by our framework. We also note that the situation where there is no competing flow in a queueing system frequently happens in the cellular base station because most modern base stations create a virtual individual queue, called \textit{bearer}, upon reception of a flow toward a cellular device (i.e., a remote machine in this scenario)~\cite{drwa2016}. The virtual queues in a base station do not interfere each other, so the queueing in the virtual queue is mostly self-induced. 

In the following section, we will provide separate analyses for two branches where $T^{on}_{k}$ is homogeneous irrespective of $k$ or $T^{on}_{k}$ is all heterogeneous. 

\begin{figure}[!t]
	\centering
	\includegraphics[width=0.95\columnwidth]{figs/caseonoff.pdf}
    \caption{A depiction of the packet arrival behavior over time in the on and off traffic generation model.}	
    \label{fig:caseonoff}
\end{figure}

\noindent{\bf{High and Low Traffic Generation Model:}}
With this model, we emulate the case where a low-latency service user intermittently creates control toward a remote machine while a background media stream such as video or audio session persists over time. We expect this pattern of traffic generation will frequently occur in the AR or MR type of services, in which the users need to transmit their multimedia information along with their control information with latency guarantee so that the server system can manipulate or augment the multimedia data and return the data to the user with nearly unnoticeable delay. We capture such a persistent background stream with the rate of $\lambda^{L}_k$ and its merged stream with intermittent control packets as $\lambda^{H}_k$, where $H$ and $L$ stand for high and low. This model is depicted in Fig.~\ref{fig:casehighlow}. We will later discuss two branches: homogeneous and heterogeneous $\lambda^{H}_k$ over $k$, while $\lambda^{L}_k$ is intentionally being homogeneous irrespective of $k$ because it represents a media stream.


\begin{figure}[!t]
	\centering
	\includegraphics[width=0.95\columnwidth]{figs/casehighlow.pdf}
    \caption{A depiction of the packet arrival behavior over time in the high and low traffic generation model.}	
    \label{fig:casehighlow}
\end{figure}
